Closing a Source Complexity Gap between Chapel and HPX

A previous case study measured performance vs source-code complexity across multiple languages. The case study identified Chapel and HPX provide similar performance and code complexity. This paper is the result of initial steps toward closing the source-code complexity gap between Chapel and HPX by using a source-to-source compiler. The investigation assesses the single-machine performance of both Chapel and Chplx applications across Arm and x86.

==> figs.tex <==
\begin{figure}[tb]
\begin{tikzpicture}

\begin{axis}[grid,xlabel={Gigabytes},ylabel=
{Seconds},legend style={at={(0.5,-0.2)},anchor=north},legend columns=4]
%{Rate},xmin=1,xmax=32, legend pos=north east]

    %\addplot[black,thick,mark=square*] table [x expr=\thisrowno{0},y expr=\thisrowno{1}, col sep=comma] {summer/chapel_stream_copy.csv};
    %\addplot[blue,thick,mark=diamond*] table [x expr=\thisrowno{0},y expr=\thisrowno{1}, col sep=comma] {summer/chplx_stream_copy.csv};

    %\addplot[black,thick,mark=square*] table [x expr=\thisrowno{0},y expr=\thisrowno{1}, col sep=comma] {summer/chapel_stream_add.csv};
    %\addplot[blue,thick,mark=diamond*] table [x expr=\thisrowno{0},y expr=\thisrowno{1}, col sep=comma] {summer/chplx_stream_add.csv};

    %\addplot[black,thick,mark=square*] table [x expr=\thisrowno{0},y expr=\thisrowno{1}, col sep=comma] {summer/chapel_stream_scale.csv};
    %\addplot[blue,thick,mark=diamond*] table [x expr=\thisrowno{0},y expr=\thisrowno{1}, col sep=comma] {summer/chplx_stream_scale.csv};

    %\addplot[black,thick,mark=square*] table [x expr=\thisrowno{0},y expr=\thisrowno{1}, col sep=comma] {summer/chapel_stream_triad.csv};
    %\addplot[blue,thick,mark=diamond*] table [x expr=\thisrowno{0},y expr=\thisrowno{1}, col sep=comma] {summer/chplx_stream_triad.csv};

    %\addplot[black,thick,mark=square*] table [x expr=\thisrowno{0},y expr=\thisrowno{1}, col sep=comma] {summer/chapel_stream_copy_rate.csv};
    %\addplot[blue,thick,mark=diamond*] table [x expr=\thisrowno{0},y expr=\thisrowno{1}, col sep=comma] {summer/chplx_stream_copy_rate.csv};

    %\addplot[black,thick,mark=square*] table [x expr=\thisrowno{0},y expr=\thisrowno{1}, col sep=comma] {summer/chapel_stream_add_rate.csv};
    %\addplot[blue,thick,mark=diamond*] table [x expr=\thisrowno{0},y expr=\thisrowno{1}, col sep=comma] {summer/chplx_stream_add_rate.csv};

    %\addplot[black,thick,mark=square*] table [x expr=\thisrowno{0},y expr=\thisrowno{1}, col sep=comma] {summer/chapel_stream_scale_rate.csv};
    %\addplot[blue,thick,mark=diamond*] table [x expr=\thisrowno{0},y expr=\thisrowno{1}, col sep=comma] {summer/chplx_stream_scale_rate.csv};

    %\addplot[black,thick,mark=square*] table [x expr=\thisrowno{0},y expr=\thisrowno{1}, col sep=comma] {summer/chapel_stream_triad_rate.csv};
    %\addplot[blue,thick,mark=diamond*] table [x expr=\thisrowno{0},y expr=\thisrowno{1}, col sep=comma] {summer/chplx_stream_triad_rate.csv};
    
    %\addplot[black,thick,mark=square*] table [x expr=\thisrowno{4},y expr=\thisrowno{6}, col sep=comma] {summer/chpl_gups_final_data_scaling.csv};
    %\addplot[blue,thick,mark=diamond*] table [x expr=\thisrowno{4},y expr=\thisrowno{6}, col sep=comma] {summer/chplx_gups_final_data_scaling.csv};
    

    %\addplot[black,thick,mark=square*] table [x expr=\thisrowno{5},y expr=\thisrowno{2}, col sep=comma] {summer/chpl_gups_final_data_scaling.csv};
    %\addplot[blue,thick,mark=diamond*] table [x expr=\thisrowno{5},y expr=\thisrowno{2}, col sep=comma] {summer/chplx_gups_final_data_scaling.csv};

    \addplot[black,thick,mark=square*] table [x expr=\thisrowno{0},y expr=\thisrowno{1}, col sep=comma] {summer/chpl_stream_copy_data_scaling.csv};
    \addplot[black,thick,mark=diamond*] table [x expr=\thisrowno{0},y expr=\thisrowno{1}, col sep=comma] {summer/chpl_stream_add_data_scaling.csv};
    \addplot[black,thick,mark=*] table [x expr=\thisrowno{0},y expr=\thisrowno{1}, col sep=comma] {summer/chpl_stream_scale_data_scaling.csv};
    \addplot[black,thick,mark=triangle*] table [x expr=\thisrowno{0},y expr=\thisrowno{1}, col sep=comma] {summer/chpl_stream_triad_data_scaling.csv};

    \addplot[gray,thick,mark=square*] table [x expr=\thisrowno{0},y expr=\thisrowno{1}, col sep=comma] {summer/chplx_stream_copy_data_scaling.csv};
    \addplot[gray,thick,mark=diamond*] table [x expr=\thisrowno{0},y expr=\thisrowno{1}, col sep=comma] {summer/chplx_stream_add_data_scaling.csv};
    \addplot[gray,thick,mark=*] table [x expr=\thisrowno{0},y expr=\thisrowno{1}, col sep=comma] {summer/chplx_stream_scale_data_scaling.csv};
    \addplot[gray,thick,mark=triangle*] table [x expr=\thisrowno{0},y expr=\thisrowno{1}, col sep=comma] {summer/chplx_stream_triad_data_scaling.csv};

    \legend{chpl-copy,chpl-add,chpl-scale,chpl-triad,chplx-copy,chplx-add,chplx-scale,chplx-triad};

\end{axis}
\end{tikzpicture}
    \caption{STREAM Copy, Add, Scale, Triad Data Scaling w/32 threads}
    \label{fig:performance:streamDataScaling}
\end{figure}
